Scalable Load Balancing Algorithms in Networked Systems

A fundamental challenge in large-scale networked systems viz., data centers and cloud networks is to distribute tasks to a pool of servers, using minimal instantaneous state information, while providing excellent delay performance. In this thesis we design and analyze load balancing algorithms that aim to achieve a highly efficient distribution of tasks, optimize server utilization, and minimize communication overhead.

==> threshold.tex <==

\begin{abstract}
We consider a system of $N$~identical parallel server pools and a single
dispatcher where tasks arrive as a Poisson process of rate $\lambda(N)$.
Arriving tasks cannot be queued, and must immediately be assigned
to one of the server pools to start execution.
The execution times are assumed to be exponentially distributed with
unit mean, and do not depend on the number of tasks contending for service.


When a task arrives, the dispatcher assigns it to an arbitrary
server pool with fewer than $L$~active tasks, if there is any, to
an arbitrary server pool with fewer than $H \geq L$ tasks otherwise, or to
a randomly selected server pool if all server pools have $H$ or more tasks.
This threshold-based scheme can be implemented in a server-driven manner,
with only O($1$) communication overhead per task.

We derive the fluid limit for the system occupancy process in the
regime $\lambda(N) / N \to \lambda$ as $N\to\infty$, along with the
associated fixed point.
We show that the fixed point coincides with that for the JSQ policy
in case $L = \lfloor \lambda \rfloor$ and $H = L + 1$
indicating that fluid-level optimality in stationarity can be achieved
with only O($1$) communication overhead per task,
as opposed to O($N$) in the JSQ policy.
We further establish that in case $L = \lfloor \lambda \rfloor$
and  $H = L + 1$
the diffusion limit also corresponds
to that for the Join the Shortest Queue policy, implying that diffusion-level optimality
can be obtained with only O($1$) communication overhead per task as well.
\end{abstract}

\section{Introduction}

In the present chapter we establish fluid and diffusion limits for
threshold-based load balancing schemes in large-scale systems.
Specifically, we consider 
a family of threshold-based schemes referred to as $T(L, H)$ where
the assignment of tasks is guided by two threshold parameters~$H$ and~$L$.
Incoming tasks are dispatched to an arbitrary server
pool with fewer than $L$~active tasks, if there is any, to an arbitrary
server pool with fewer than $H > L$ tasks otherwise, or to a randomly
selected server pool if all server pools have $H$ or more tasks.
Such a scheme can be implemented in a server-driven manner,
with $O(1)$ communication overhead per task,
as opposed to $O(d)$ in the power-of-$d$ scheme.
It is worth observing that for $L = 1$ and $H = 1$ or $H = \infty$ the
threshold-based scheme reduces to the so-called Join-the-Idle-Queue
(JIQ) policy as considered in Chapter~\ref{chap:jiq}.
We consider a regime where the number of servers~$N$ grows large,
and for convenience we assume a Poisson arrival process of rate
$\lambda(N)$ and unit-mean exponential service requirements.
We derive the fluid limit for the system occupancy process in the regime
$\lambda(N) / N \to \lambda>0$ as $N\to\infty$, along with the associated
fixed point.
Furthermore, observe that in  the threshold-based schemes,  the assignment
probabilities for incoming tasks to a server with a specific number of 
active tasks may depend on variables that are not
visible in the fluid-scaled system occupancy state.
As a result, the conventional machinery for establishing fluid limits
as described in~\cite{EK2009, K70, K71} and used in~\cite{Mitzenmacher01} does not
apply. 
We leverage the time-scale separation technique in~\cite{HK94} to get
the fluid limit in this scenario.
We show that the fixed point of the
fluid limit coincides with that for the JSQ policy in case
$L = \lfloor \lambda \rfloor$ and  $H = L + 1$
indicating that fluid-level optimality in stationarity can be achieved
with only O($1$) overhead per task, as opposed to O($N$) in the JSQ policy.
We further establish that in case $L = \lfloor \lambda \rfloor$
and $H = L + 1$
the diffusion limit also corresponds
to that for the JSQ policy, implying that diffusion-level optimality
can be obtained with only O($1$) overhead per task as well.
As mentioned earlier, for $L = 1$ and $H = 1$ or $H = \infty$ the
threshold-based scheme corresponds to the so-called JIQ policy.
The fluid-level and diffusion-level optimality properties of the
threshold-based scheme with only O($1$) overhead per task are in fact
reminiscent of findings for JIQ-type policies in a queueing
scenario as in Chapter~\ref{chap:jiq}.



\paragraph*{Organization.}
The remainder of the chapter is organized as follows.
In Section~\ref{sec:model-descr-thres} we present a detailed model
description and state the main results.
